Long-short Term Motion Feature for Action Classification and Retrieval

We propose a method for representing motion information for video classification and retrieval. We improve upon local descriptor based methods that have been among the most popular and successful models for representing videos. The desired local descriptors need to satisfy two requirements: 1) to be representative, 2) to be discriminative. Therefore, they need to occur frequently enough in the videos and to be be able to tell the difference among different types of motions. To generate such local descriptors, the video blocks they are based on must contain just the right amount of motion information. However, current state-of-the-art local descriptor methods use video blocks with a single fixed size, which is insufficient for covering actions with varying speeds. In this paper, we introduce a long-short term motion feature that generates descriptors from video blocks with multiple lengths, thus covering motions with large speed variance. Experimental results show that, albeit simple, our model achieves state-of-the-arts results on several benchmark datasets.

==> backup.tex <==
The interest in Content based video retrieval system is increasing because of the explosive growth of both user and automatically generated videos, as well as the inherent limitations in metadata-based systems. The performance of content based video retrieval system greatly relies on the features to represent videos. Due to the grate demand of memory and computational requirement, most video description algorithms adopt local feature scheme, that is: 1) , i.e., cubiods or trajectories; 2) ; 3) aggregate the descriptors together to generate a video description. For example, STIP consists in detecting sparse spatio-temporal interest points, which are then described using local spatio-temporal features: Histogram of Oriented Gradients (HOG)  and Histogram of Optical Flow (HOF) and aggregated using pooling methods such as Bag Of Features (BoF) or Fisher Vector. Dense Trajectory makes use of dense trajectories, which are described by HOG, HOF, and Motion Boundary Histogram (MBH) and again aggregated by BoF or Fisher vector. State-of-art approaches shows that having local descriptors across multiple succession frames (L>1) generally works better than between a pair of frames,  Generally speaking, short-term motion (small L) information is easier to locate while long-term motion (large L) information is more discriminative. However, choosing an optimal L is data dependent and different for different algorithms, i.e., [1] shows that 15 frames work best across several datasets, [2] generates features from a secession of 10 frames. In this paper, we propose to use multiple L to capture both long term and short term information. 

